Gradient Scan Gibbs Sampler: an efficient algorithm for high-dimensional Gaussian distributions

This paper deals with Gibbs samplers that include high dimensional conditional Gaussian distributions. It proposes an efficient algorithm that avoids the high dimensional Gaussian sampling and relies on a random excursion along a small set of directions. The algorithm is proved to converge, i.e. the drawn samples are asymptotically distributed according to the target distribution. Our main motivation is in inverse problems related to general linear observation models and their solution in a hierarchical Bayesian framework implemented through sampling algorithms. It finds direct applications in semi-blind/unsupervised methods as well as in some non-Gaussian methods. The paper provides an illustration focused on the unsupervised estimation for super-resolution methods.

==> alphabet.tex <==
% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\RequirePackage{amsmath}
\RequirePackage{bbm}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

% 

\def\sbm#1{\mathbf{#1}}                % Style gras italique (necessite amsmath)           
\def\sbmm#1{\boldsymbol{#1}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\mathrm{#1}}               % Style droit en math
\def\sbv#1{\mathbf{#1}}               % Style gras droit
\def\scu#1{\mathcal{#1\XS}}           % Style cursif
\def\scb#1{\boldsymbol{\mathcal{#1}}} % Style gras cursif
\def\sbl#1{\mathbbm{#1}}              % Style blackboard (necessite bbm)

% 

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}}  \def\ab{{\sbm{a}}}
\def\Bb{{\sbm{B}}}  \def\bb{{\sbm{b}}}
\def\Cb{{\sbm{C}}}  \def\cb{{\sbm{c}}}
\def\Db{{\sbm{D}}}  \def\db{{\sbm{d}}}
\def\Eb{{\sbm{E}}}  \def\eb{{\sbm{e}}}
\def\Fb{{\sbm{F}}}  \def\fb{{\sbm{f}}}
\def\Gb{{\sbm{G}}}  \def\gb{{\sbm{g}}}
\def\Hb{{\sbm{H}}}  \def\hb{{\sbm{h}}}
\def\Ib{{\sbm{I}}}  \def\ib{{\sbm{i}}}
\def\Jb{{\sbm{J}}}  \def\jb{{\sbm{j}}}
\def\Kb{{\sbm{K}}}  \def\kb{{\sbm{k}}}
\def\Lb{{\sbm{L}}}  \def\lb{{\sbm{l}}}
\def\Mb{{\sbm{M}}}  \def\mb{{\sbm{m}}}
\def\Nb{{\sbm{N}}}  \def\nb{{\sbm{n}}}
\def\Ob{{\sbm{O}}}  \def\ob{{\sbm{o}}}
\def\Pb{{\sbm{P}}}  \def\pb{{\sbm{p}}}
\def\Qb{{\sbm{Q}}}  \def\qb{{\sbm{q}}}
\def\Rb{{\sbm{R}}}  \def\rb{{\sbm{r}}}
\def\Sb{{\sbm{S}}}  \def\sb{{\sbm{s}}}
\def\Tb{{\sbm{T}}}  \def\tb{{\sbm{t}}}
\def\Ub{{\sbm{U}}}  \def\ub{{\sbm{u}}}
\def\Vb{{\sbm{V}}}  \def\vb{{\sbm{v}}}
\def\Wb{{\sbm{W}}}  \def\wb{{\sbm{w}}}
\def\Xb{{\sbm{X}}}  \def\xb{{\sbm{x}}}
\def\Yb{{\sbm{Y}}}  \def\yb{{\sbm{y}}}
\def\Zb{{\sbm{Z}}}  \def\zb{{\sbm{z}}}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}}   \def\Acb{{\scb{A}}}
\def\Bc{{\scu{B}}}   \def\Bcb{{\scb{B}}}
\def\Cc{{\scu{C}}}   \def\Ccb{{\scb{C}}}
\def\Dc{{\scu{D}}}   \def\Dcb{{\scb{D}}}
\def\Ec{{\scu{E}}}   \def\Ecb{{\scb{E}}}
\def\Fc{{\scu{F}}}   \def\Fcb{{\scb{F}}}
\def\Gc{{\scu{G}}}   \def\Gcb{{\scb{G}}}
\def\Hc{{\scu{H}}}   \def\Hcb{{\scb{H}}}
\def\Ic{{\scu{I}}}   \def\Icb{{\scb{I}}}
\def\Jc{{\scu{J}}}   \def\Jcb{{\scb{J}}}
\def\Kc{{\scu{K}}}   \def\Kcb{{\scb{K}}}
\def\Lc{{\scu{L}}}   \def\Lcb{{\scb{L}}}
\def\Mc{{\scu{M}}}   \def\Mcb{{\scb{M}}}
\def\Nc{{\scu{N}}}   \def\Ncb{{\scb{N}}}
\def\Oc{{\scu{O}}}   \def\Ocb{{\scb{O}}}
\def\Pc{{\scu{P}}}   \def\Pcb{{\scb{P}}}
\def\Qc{{\scu{Q}}}   \def\Qcb{{\scb{Q}}}
\def\Rc{{\scu{R}}}   \def\Rcb{{\scb{R}}}
\def\Sc{{\scu{S}}}   \def\Scb{{\scb{S}}}
\def\Tc{{\scu{T}}}   \def\Tcb{{\scb{T}}}
\def\Uc{{\scu{U}}}   \def\Ucb{{\scb{U}}}
\def\Vc{{\scu{V}}}   \def\Vcb{{\scb{V}}}
\def\Wc{{\scu{W}}}   \def\Wcb{{\scb{W}}}
\def\Xc{{\scu{X}}}   \def\Xcb{{\scb{X}}}
\def\Yc{{\scu{Y}}}   \def\Ycb{{\scb{Y}}}
\def\Zc{{\scu{Z}}}   \def\Zcb{{\scb{Z}}}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}}  \def\aD{{\sdm{a}}}
\def\BD{{\sdm{B}}}  \def\bD{{\sdm{b}}}
\def\CD{{\sdm{C}}}  \def\cD{{\sdm{c}}}
\def\DD{{\sdm{D}}}  \def\dD{{\sdm{d}}}
\def\ED{{\sdm{E}}}  \def\eD{{\sdm{e}}}
\def\FD{{\sdm{F}}}  \def\fD{{\sdm{f}}}
\def\GD{{\sdm{G}}}  \def\gD{{\sdm{g}}}
\def\HD{{\sdm{H}}}  \def\hD{{\sdm{h}}}
\def\ID{{\sdm{I}}}  \def\iD{{\sdm{i}}}
\def\JD{{\sdm{J}}}  \def\jD{{\sdm{j}}}
\def\KD{{\sdm{K}}}  \def\kD{{\sdm{k}}}
\def\LD{{\sdm{L}}}  \def\lD{{\sdm{l}}}
\def\MD{{\sdm{M}}}  \def\mD{{\sdm{m}}}
\def\ND{{\sdm{N}}}  \def\nD{{\sdm{n}}}
\def\OD{{\sdm{O}}}  \def\oD{{\sdm{o}}}
\def\PD{{\sdm{P}}}  \def\pD{{\sdm{p}}}
\def\QD{{\sdm{Q}}}  \def\qD{{\sdm{q}}}
\def\RD{{\sdm{R}}}  \def\rD{{\sdm{r}}}
\def\SD{{\sdm{S}}}  \def\sD{{\sdm{s}}}
\def\TD{{\sdm{T}}}  \def\tD{{\sdm{t}}}
\def\UD{{\sdm{U}}}  \def\uD{{\sdm{u}}}
\def\VD{{\sdm{V}}}  \def\vD{{\sdm{D}}}
\def\WD{{\sdm{W}}}  \def\wD{{\sdm{w}}}
\def\XD{{\sdm{X}}}  \def\xD{{\sdm{x}}}
\def\YD{{\sdm{Y}}}  \def\yD{{\sdm{y}}}
\def\ZD{{\sdm{Z}}}  \def\zD{{\sdm{z}}}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}}  \def\av{{\sbv{a}}}
\def\Bv{{\sbv{B}}}  \def\bv{{\sbv{b}}}
\def\Cv{{\sbv{C}}}  \def\cv{{\sbv{c}}}
\def\Dv{{\sbv{D}}}  \def\dv{{\sbv{d}}}
\def\Ev{{\sbv{E}}}  \def\ev{{\sbv{e}}}
\def\Fv{{\sbv{F}}}  \def\fv{{\sbv{f}}}
\def\Gv{{\sbv{G}}}  \def\gv{{\sbv{g}}}
\def\Hv{{\sbv{H}}}  \def\hv{{\sbv{h}}}
\def\Iv{{\sbv{I}}}  \def\iv{{\sbv{i}}}
\def\Jv{{\sbv{J}}}  \def\jv{{\sbv{j}}}
\def\Kv{{\sbv{K}}}  \def\kv{{\sbv{k}}}
\def\Lv{{\sbv{L}}}  \def\lv{{\sbv{l}}}
\def\Mv{{\sbv{M}}}  \def\mv{{\sbv{m}}}
\def\Nv{{\sbv{N}}}  \def\nv{{\sbv{n}}}
\def\Ov{{\sbv{O}}}  \def\ov{{\sbv{o}}}
\def\Pv{{\sbv{P}}}  \def\pv{{\sbv{p}}}
\def\Qv{{\sbv{Q}}}  \def\qv{{\sbv{q}}}
\def\Rv{{\sbv{R}}}  \def\rv{{\sbv{r}}}
\def\Sv{{\sbv{S}}}  \def\sv{{\sbv{s}}}
\def\Tv{{\sbv{T}}}  \def\tv{{\sbv{t}}}
\def\Uv{{\sbv{U}}}  \def\uv{{\sbv{u}}}
\def\Vv{{\sbv{V}}}  \def\vv{{\sbv{v}}}
\def\Wv{{\sbv{W}}}  \def\wv{{\sbv{w}}}
\def\Xv{{\sbv{X}}}  \def\xv{{\sbv{x}}}
\def\Yv{{\sbv{Y}}}  \def\yv{{\sbv{y}}}
\def\Zv{{\sbv{Z}}}  \def\zv{{\sbv{z}}}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}}  \def\abb{{\sbl{a}}}
\def\Bbb{{\sbl{B}}}  \def\bbb{{\sbl{b}}}
\def\Cbb{{\sbl{C}}}  \def\cbb{{\sbl{c}}}
\def\Dbb{{\sbl{D}}}  \def\dbb{{\sbl{d}}}
\def\Ebb{{\sbl{E}}}  \def\ebb{{\sbl{e}}}
\def\Fbb{{\sbl{F}}}  \def\fbb{{\sbl{f}}}
\def\Gbb{{\sbl{G}}}  \def\gbb{{\sbl{g}}}
\def\Hbb{{\sbl{H}}}  \def\hbb{{\sbl{h}}}
\def\Ibb{{\sbl{I}}}  \def\ibb{{\sbl{i}}}
\def\Jbb{{\sbl{J}}}  \def\jbb{{\sbl{j}}}
\def\Kbb{{\sbl{K}}}  \def\kbb{{\sbl{k}}}
\def\Lbb{{\sbl{L}}}  \def\lbb{{\sbl{l}}}
\def\Mbb{{\sbl{M}}}  \def\mbb{{\sbl{m}}}
\def\Nbb{{\sbl{N}}}  \def\nbb{{\sbl{n}}}
\def\Obb{{\sbl{O}}}  \def\obb{{\sbl{o}}}
\def\Pbb{{\sbl{P}}}  \def\pbb{{\sbl{p}}}
\def\Qbb{{\sbl{Q}}}  \def\qbb{{\sbl{q}}}
\def\Rbb{{\sbl{R}}}  \def\rbb{{\sbl{r}}}
\def\Sbb{{\sbl{S}}}  \def\sbb{{\sbl{s}}}
\def\Tbb{{\sbl{T}}}  \def\tbb{{\sbl{t}}}
\def\Ubb{{\sbl{U}}}  \def\ubb{{\sbl{u}}}
\def\Vbb{{\sbl{V}}}  \def\vbb{{\sbl{v}}}
\def\Wbb{{\sbl{W}}}  \def\wbb{{\sbl{w}}}
\def\Xbb{{\sbl{X}}}  \def\xbb{{\sbl{x}}}
\def\Ybb{{\sbl{Y}}}  \def\ybb{{\sbl{y}}}
\def\Zbb{{\sbl{Z}}}  \def\zbb{{\sbl{z}}}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}}
\def\betab       {{\sbmm{\beta}}}
\def\gammab      {{\sbmm{\gamma}}}      \def\Gammab    {{\sbmm{\Gamma}}}
\def\deltab      {{\sbmm{\delta}}}      \def\Deltab    {{\sbmm{\Delta}}}
\def\epsilonb    {{\sbmm{\epsilon}}}
\def\varepsilonb {{\sbmm{\varepsilon}}}
\def\etab        {{\sbmm{\eta}}}
\def\thetab      {{\sbmm{\theta}}}      \def\Thetab    {{\sbmm{\Theta}}}
\def\varthetab   {{\sbmm{\vartheta}}}
\def\iotab       {{\sbmm{\iota}}}
\def\kappab      {{\sbmm{\kappa}}}
\def\varkappab   {{\sbmm{\varkappa}}}
\def\lambdab     {{\sbmm{\lambda}}}     \def\Lambdab   {{\sbmm{\Lambda}}}
\def\mub         {{\sbmm{\mu}}}
\def\nub         {{\sbmm{\nu}}}
\def\xib         {{\sbmm{\xi}}}         \def\Xib       {{\sbmm{\Xi}}}
\def\pib         {{\sbmm{\pi}}}         \def\Pib       {{\sbmm{\Pi}}}
\def\varpib      {{\sbmm{\varpi}}}
\def\rhob        {{\sbmm{\rho}}}
\def\varrhob     {{\sbmm{\varrho}}}
\def\sigmab      {{\sbmm{\sigma}}}      \def\Sigmab    {{\sbmm{\Sigma}}}
\def\varsigmab   {{\sbmm{\varsigma}}}   \def\Varsigmab {{\sbmm{\Varsigma}}}
\def\phib        {{\sbmm{\phi}}}        \def\Phib      {{\sbmm{\Phi}}}
\def\varphib     {{\sbmm{\varphi}}}
\def\chib        {{\sbmm{\chi}}}
\def\psib        {{\sbmm{\psi}}}        \def\Psib      {{\sbmm{\Psi}}}
\def\omegab      {{\sbmm{\omega}}}      \def\Omegab    {{\sbmm{\Omega}}}
\def\taub        {{\sbmm{\tau}}}
\def\upsilonb    {{\sbmm{\upsilon}}}   \def\Upsilonb  {{\sbmm{\Upsilon}}}
\def\zetab       {{\sbmm{\zeta}}}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}}        \def\zerobb   {{\sbl{O}}}
\def\unb     {{\sbv{1}}}        \def\unbb     {{\sbl{1}}}
\def\deuxb   {{\sbv{2}}}        \def\deuxbb   {{\sbl{2}}}
\def\troisb  {{\sbv{3}}}        \def\troisbb  {{\sbl{3}}}
\def\quatreb {{\sbv{4}}}        \def\quatrebb {{\sbl{4}}}
\def\cinqb   {{\sbv{5}}}        \def\cinqbb   {{\sbl{5}}}
\def\sixb    {{\sbv{6}}}        \def\sixbb    {{\sbl{6}}}
\def\septb   {{\sbv{7}}}        \def\septbb   {{\sbl{7}}}
\def\huitb   {{\sbv{8}}}        \def\huitbb   {{\sbl{8}}}
\def\neufb   {{\sbv{9}}}        \def\neufbb   {{\sbl{9}}}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

% ALPHABET GAUTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}}  \def\ag{{\textgoth{a}}}
\def\Bg{{\textgoth{B}}}  \def\bg{{\textgoth{b}}}
\def\Cg{{\textgoth{C}}}  \def\cg{{\textgoth{c}}}
\def\Dg{{\textgoth{D}}}  \def\dg{{\textgoth{d}}}
\def\Eg{{\textgoth{E}}}  \def\eg{{\textgoth{e}}}
\def\Fg{{\textgoth{F}}}  \def\fg{{\textgoth{f}}}
\def\Gg{{\textgoth{G}}}  %\def\gg{{\textgoth{g}}}
\def\Hg{{\textgoth{H}}}  \def\hg{{\textgoth{h}}}
\def\Ig{{\textgoth{I}}}  \def\ig{{\textgoth{i}}}
\def\Jg{{\textgoth{J}}}  \def\jg{{\textgoth{j}}}
\def\Kg{{\textgoth{K}}}  \def\kg{{\textgoth{k}}}
\def\Lg{{\textgoth{L}}}  \def\lg{{\textgoth{l}}}
\def\Mg{{\textgoth{M}}}  \def\mg{{\textgoth{m}}}
\def\Ng{{\textgoth{N}}}  \def\ng{{\textgoth{n}}}
\def\Og{{\textgoth{O}}}  \def\og{{\textgoth{o}}}
\def\Pg{{\textgoth{P}}}  \def\pg{{\textgoth{p}}}
\def\Qg{{\textgoth{Q}}}  \def\qg{{\textgoth{q}}}
\def\Rg{{\textgoth{R}}}  \def\rg{{\textgoth{r}}}
\def\Sg{{\textgoth{S}}}  \def\sg{{\textgoth{s}}}
\def\Tg{{\textgoth{T}}}  \def\tg{{\textgoth{t}}}
\def\Ug{{\textgoth{U}}}  \def\ug{{\textgoth{u}}}
\def\Vg{{\textgoth{V}}}  \def\vg{{\textgoth{v}}}
\def\Wg{{\textgoth{W}}}  \def\wg{{\textgoth{w}}}
\def\Xg{{\textgoth{X}}}  \def\xg{{\textgoth{x}}}
\def\Yg{{\textgoth{Y}}}  \def\yg{{\textgoth{y}}}
\def\Zg{{\textgoth{Z}}}  \def\zg{{\textgoth{z}}}

